Disentangling Syntax and Semantics in the Brain with Deep Networks

The activations of language transformers like GPT-2 have been shown to linearly map onto brain activity during speech comprehension. However, the nature of these activations remains largely unknown and presumably conflate distinct linguistic classes. Here, we propose a taxonomy to factorize the high-dimensional activations of language models into four combinatorial classes: lexical, compositional, syntactic, and semantic representations. We then introduce a statistical method to decompose, through the lens of GPT-2's activations, the brain activity of 345 subjects recorded with functional magnetic resonance imaging (fMRI) during the listening of ~4.6 hours of narrated text. The results highlight two findings. First, compositional representations recruit a more widespread cortical network than lexical ones, and encompass the bilateral temporal, parietal and prefrontal cortices. Second, contrary to previous claims, syntax and semantics are not associated with separated modules, but, instead, appear to share a common and distributed neural substrate. Overall, this study introduces a versatile framework to isolate, in the brain activity, the distributed representations of linguistic constructs.

==> charlotte_discussion_short.tex <==
Here, we introduced a method to extract syntactic representations from deep neural language models, allowing us to decompose the brain activity of 345 subjects reading narratives into their lexical, compositional, syntactic and semantic representations. We found that 

% past work
Past work use overall difference in activations:
    at the lexical level:
        Friederici et al (Segregating semantic and syntactic aspects of processing in the human brain: an fMRI investigation of different word types)

    at the compositional level:
        Pallier, et al, PNAS 2011: 
            - fMRI
            - use isolated sentences with varying constituent sizes
            - use French and Jabberwocky sentences 
            - main conclusion: dissociated regions for syntax (broca) and semantics (STG)
            
        Fedorenko et al 2012, neuropsychogia (Lexical and syntactic representations in the brain: An fMRI investigation with multi-voxel pattern analyses)
            - fMRI
            - use english and jabberwocky
            - main conclusion: same regions for syntax and semantics (distributed representations
        
        Similar work using intracranial: Fedorenko et al (Neural correlate of the construction of sentence meaning)

Recent work on the sentence/word level modeling (i.e. brain correlation across words/sentences, not brain average activation between 2 conditions):
    with "symbolic" features:
        Syntax:
            Brennan & Pylkannen: MEG Evidence for Incremental Sentence Composition in the AnteriorTemporal Lobe 
                - MEG, correlate with syntactic trees
            Nelson, et al & Dehaene PNAS 2018
                - intracranial EEG, correlate brain response to end of constituents
            
    with partially interpretable model
        Brennan et al: Finding syntax in human encephalography with beam search
            - EEG, correlate with merge operation
        Recent Leila Wehbe arXiv paper on the embedding of syntactic trees
    
    With fully distributed models:
        word: 
            Tom Mitchell's science paper (2008?) on fmri + word embeddings 
            Huth et al Nature 2016: fMRI + word embeddings (attempt to interpret semantics dimensions, but only find that the first two are sort of interpretable)
        syntax: recent leila wehbe paper
        unspecified correlation: 
            every fMRI/MEG GPT2 correlation
            huth neurips
            wehbe's papers
            king caucheteux
            schrimpf fedorenko et al

% Contributions of the paper
1. method: first modeling of distributed syntactic representations
    - applies to natural data (cite Huth's paper : "the revolution will not be controlled"
    - no need to use questionable stimuli (jabberwocky)
    - conceptually: we shuffle the stimuli (like Lehrer et al , Journal of neruoscience, scramblind paragraphes and sentences breaks the correlations between subjects), not the features (as one would do with a permutation test using an explicit feature).
    
2. result: 
    - compare cortical distributions: overall, in favor of distributed representations, similar brain regions share syntactic and semantic representations

Limits
    - fmri: slow response, bad SNR, average across subjects, weird narratives
    - semantics is poorly defined (as usual)
    - syntactic representations are not dissected:
        + role of memory load
        + syntactic representations (the tree) != syntactic operations (the building of the tree)
    - shuffling relies on a symbolic linguistic model: the dependency tree



%Neuroscience : decompose the language network
\textbf{Decomposing natural language processing into syntax and semantics}


Results and previous work:
\begin{itemize}
\item Replicated previous results: compositional semantics 
\item \undeline{Syntax vs. semantics} (first row vs second row). Syntax involves a temporal network, superior temporal and Wernicke. Semantics, on the contrary, more in the temporal Lobe, Broca area, and Wernicke. 
\item \undeline{Lexical vs compositional}: Weheb, Huth, more distributed network, in both hemispheres. 
\item \undeline{Lexical semantic and lexical syntax}: lower scores. Yet, Wernicke present, and temporal for semantic (XXXX). Do not include Broca. May be due to highly restrictive concatenation setting. We preferred to be restrictive.  
\item \undeline{Focus on compositional semantics}: more distributed and strong response. 
\item \undeline{Lexical syntax} ? 
\end{itemize}

Conclusions and limits:

From these results, we argue that we can decompose language in the brain into nine types of linguistic processes. 
First, we acknowledge the limits of our taxonomy. Semantics is here defined as the non-syntactic representations in the brain that can be explained by the activations of GPT2. 

\begin{itemize}
    \item Taxonomy. Semantics : a large acceptance, which can be discussed. Can contain other elements such as emotions. Emotions are an interesting case because. 
    \item Taxonomy. Lexical. Question of what is the “lexicon”. Sublexical ? At the word level. BPE biais ? Here more than 99.5\% of words (not BPE). 
    \item Very strong assumption about the GPT2. We consider that GPT2 activations the whole semantic and syntactic information about language in the brain. There are clues in the literature that it can reach the noise ceiling. But difficult to prove. Precise: decompose GPT2-type language representations in the brain. 
    \item fMRI encoding method. limits: Multi-subjects, low scores. Temporal resolution of fMRI. FIR. Mlit-subjects => better signal-to-noise ratio. BUT ignore individual effects. 

\end{itemize}
\textbf{Better understanding the linkns between NLM and the brain}

We show that intermediate stages of computations share similarities. 
Replicate previous findings about layer decomposition (middle layers predict). Other research studies other types of decomposition: loss function (GPT2 predictive coding, Micha Heilbron, different hierarchies). In vision, in speech ().
Yet, to our knowledge, a linguistic decomposition of shared representations has not been studied NLM x brain. 


\textbf{Why this is important}

\begin{itemize}
    % General method for neuroscience
    \item In neuroscience, a common way of investigating language processing is to compare the brain activity elicited by two different controlled stimuli (e.g syntactically correct and incorrect sentences) [REF]. Due to the recording and time constraints of neuroimaging, the set of hypotheses that can be tested in one experiment is limited. Thus, different (and therefore heterogeneous) experiments focused on the neural bases of lexico-semantics [REF], compositional-syntax [REF], sentences semantics [REF], but only a few combined these different linguistic dimensions [REF]. Here, by applying a perturbation to the input space of the neural language model, it allows us to extensively test hypothesis, within a single experiment. For instance, here, we scrambled the sentences as a control. We could have tested other types of condition and compare the corresponding brain scores. 
    \item This is a general method that could be used to study other types of embeddings in the brain: in language processing (e.g. the sentiment of a sentence), but also in other deep learning areas such as vision (e.g disentangling colors and shapes by taking the expected activations of a CNN over a controlled set of inputs), and speech (e.g speaker/voice embeddings), the difficulty being to generate the set of controlled stimuli input to the deep neural network. 
     % Powerful syntactic regressor 
     \item More than the experimental setting, one faces a taxonomic obstacle when tackling the question of language processing in the brain. The concepts introduced by linguistic theories vary in the literature and mostly rely on symbolic representations (e.g. tree-like structures), which are difficult to linearly map onto brain activity [REFORMULER?]. Thus, symbols have to be (//are usually) transformed into vectors [XXX], which can have a significant influence on the experimental result [XXX] and hinder its interpretation. Here, we introduce a distributed representation that can be easily mapped onto brain activity.
     % Graph embeddings
     \item This method is part of the more general framework of graph embeddings and could be adapted for other types of symbolic structures embedded into deep neural networks activations (e.g molecules and social networks).
     %i.e generated representation symbolic structures, that goes beyond linguistics and syntax. This method requires 
     %and could be applied for other types of symbolic structures embedded into deep neural networks activations (e.g molecules and social networks). 
     %Graph embedding is an issue that goes beyond language processing and syntax. Other types of data such as social networks and molecules have an underlying symbolic structures. 
     % In Natural Language Processing, 
     \item Finally, disentangling linguistic representations is useful to increase its interpretability [XXXX PRECISER VAGUE], better control its biases [XXX FAUX?], but also to build better-performing models (e.g building semantic representations of sentences XXXX STS ?).


    

==> decomposing_old.tex <==
%Neural language models are deep neural networks trained to predict words (e.g “mat”) given their preceding context (e.g “the cat is on the [?]”), given millions of examples (e.g the Wikipedia sentences). Because they are explicit parametric models of language processing, they can be decomposed into sub-modules (e.g Transformer layer in the case of GPT2), and offer a new way of defining linguistic terms. 

\subsection{Lexicality}
Word embeddings can be considered as distributed lexical representations: 
%(from ancient greek \textit{léxis}, which is relative to the \textit{word}): 
they consist of a lookup table that associate a unique distributed representation (vector) to each word, independently of the context within which it is used.
%Word embeddings have been shown to encode many linguistic properties such as the relative locations of cities, the genre [REF]. 
In GPT2, the word embedding corresponds to the activations of the first layer $X^{(0)}$. Consequently, The lexical representations of a sentence $w \in \mathcal{V}^M$ of length $M$ (e.g "The cat is on the mat", with $M=6$) is given by:
%
\begin{align*}
\Psi_1^{(0)}(w) &= (\Psi_1^{(0)}(w)_1, \dots  \Psi_1^{(0)}(w)_M) \\ 
&= (a^{(0)}(w_1), \dots  a^{(0)}(w_M))
\end{align*}
%
Following \ref{encoding_a}, the similarity of the lexical representations between GPT2 and the brain is thus $\mathcal{R}(a^{(0)})$.

\subsection{Compositionality}
In GPT2, contextual layers (i.e. layers above the word embedding) non-linearly combine multiple words, and can thus produce representations that are more than the sum of their parts. For example, the middle layers of language transformers (e.g. layer 9 in GPT2) have been shown to (linearly) represent a variety of compositional representations such as syntactic trees [manning], co-reference [sagot?] and XXX. 
However, compositional layer can linearly propagate lexical representation, and thus correlate with brain activity solely because of a lexical similarity. 
Consequently, the similarity of the strictly compositional representations between GPT2 and the brain can be quantified by the gain in correlation observed between a compositional layer (here, layer 9) and a word-embedding layer: 

% The meaning of a sentence is generally considered to result from the combination of its individual words and
% Following the so-called Frege principle [REF], the meaning of the sentence is more than the sum of its lexical constituents (words). For instance, if some lexical components of the sentence “the cat is on the mat” are taken away (e.g. “cat” and “mat”) it remains the pseudo-sentence “the X is on the Y” (bad explanation?). 
%This residual is called compositionality. Here, we used the layer 9 of GPT2 $a^{(9)}$ to account for the holistic representation of a sentence, which has shown to encode brain activity (REF) as well as linguistic properties (Sagot). YYY (add attention mechanism here?). If language processing is the sum of lexicality and composition, the compositional representations of a sentence $x$ can be defined as the residual activations in the network, 
%\[a^{(9)}(w) - a^{(0)}(w)\] 
%and the residual explained variance in the brain : 
\begin{equation}\label{eq_comp}
    \mathcal{R}(a^{(9)}) - \mathcal{R}(a^{(0)})
\end{equation}

\subsection{Semantics}
If we assume that sentence representations strictly consist of syntax and semantics, then semantic representations are the residual representations remaining after syntactic representations have been removed. Semantic representations can thus be isolated in the brain by comparing two correlation scores: 
%
\begin{equation}\label{eq_sem}
   \mathcal{R}(a) - \mathcal{R}(\overline{a})
\end{equation}
%
with $\overline{a}$the syntactic representations extracted from $a^{(k)}$, as explained in XXX.

%Importantly, syntactic and semantic representations of $w$ can be extracted for different processing levels $k \in [0 \dots 12]$, from the lexical level of GPT2 layer $0$ to the compositional levels of GPT2's layers $1$ to $12$. Thus, equations (2), (3), (4), and (5) can be combined to build nine product features ([lexical, compositional, lexical+compositional] x [syntactic, semantic, syntactic+semantic]), including the largely studied lexico-semantics and compositional-syntactic representations (cf Figure 1).

==> equations.tex <==
\begin{align} \label{encoding_a}
\mathcal{R}^{(l)}(x) : f 
\mapsto \mathcal{L} 
\bigg( 
    f \Big(\big[ u_i \circ G^{(l)}(x)\big]_{i \in I} \Big), 
    \big( \overline{y}_i \big)_{i \in I}
    \bigg)
\end{align}

s.t

\begin{itemize}
    \item $\overline{y}$ the average brain signals:
    
        \begin{align*}
        \overline{y} & = \Big(
        \frac{1}{|\mathcal{S}|} \sum_{s \in \mathcal{S}} y_i^{(s)}
        \Big)_{i \in I}
        \end{align*}
        
    with \(y^{(s)} = (y_1^{(s)},  \dots , y_N^{(s)})\) the $N$ fMRI scans of one subject $s \in \mathcal{S}$, elicited by the story $x$
    \item \(x = (x_1,  \dots  , x_M) = (\mathrm{once}, \mathrm{upon},  \dots ., \mathrm{end.})\) the M words of the story. 
    \item \(t_x = (t_{x_1},  \dots , t_{x_M}) \in \bbR^M\)  the $M$ words' onsets and \(t_y = (t_{y_1},  \dots , t_{y_N})\) ) the timings of the $N$ scan measurements, with respect to the beginning of the experiment.
     \item $G^{(l)}(x)$, the activations of layer $l$ (\(l \in \llbracket 0, 12 \rrbracket\)) of GPT-2 when processing the full story $x$ (one vector of dimension $d$ per input word): 
     
        \begin{align*}
        G^{(l)} : \mathcal{V}^M & \rightarrow \bbR^{M \times d} \\
        x & \mapsto G^{(l)}(x) = [G^{(l)}(x)_1, \dots, G^{(l)}(x)_M]
        \end{align*}
        
    with $\mathcal{V}$ the set of vocabulary words
    \item
        The alignment functions $(u_i)_{i \in [1 \dots N]}$, used to map word features of length $M$ and time onsets $(t_{x_1}, \dots, t_{x_M})$ to fMRI scans of length $N$ and timings $(t_{y_1}, \dots, t_{y_N})$, with $N < M$. For all $i \in [1 \dots N]$, $u_i$ extracts the word features that should be mapped with the $i^{th}$ fMRI scan $y_i$, as follows:
        \begin{align*}\label{equ_align}
        u_i : \bbR^{M \times d} & \rightarrow  \bbR^{5d} \\
        z  & \mapsto 
        \big[ 
        \widetilde{ z_i}, 
        \widetilde{ z_{i-1}}, 
         \dots , 
        \widetilde{ z_{i-4}}
        \big] \\
        \widetilde{ z_i} &= \sum_{\substack{j \in \llbracket 1  \dots  M \rrbracket \\ \mathcal{T}(j) = i}} {z_j} \\
        \mathcal{T} : \llbracket 1  \dots  M \rrbracket & \rightarrow \llbracket 1  \dots   N \rrbracket \\
        j & \mapsto i \quad / \quad | t_{y_i} - t_{x_j} | = \min_{k \in \llbracket1 \dots N\rrbracket} | t_{y_k} - t_{x_j} |
        \end{align*}

\end{itemize}

==> equations_test.tex <==
\begin{align} \label{encoding_a}
\mathcal{R}^{(l)}_f(x) : \mathcal{I}(\llbracket 1 .. N \rrbracket) & \rightarrow [-1, 1] \\
I & \mapsto \mathcal{L} 
\bigg( 
    f \Big(\big( \phi_i^{(l)}(x)\big)_{i \in I} \Big), 
    \Big( \frac{1}{|\mathcal{S}|} \sum_{s \in \mathcal{S}} y_i^{(s)}\Big)_{i \in I} 
    \bigg)
\end{align}

s.t

\begin{align}\label{encoding_b}
\phi_i^{(l)}(x) & = \big[ 
\widetilde{ L^{(l)}(x)_i}, 
\widetilde{ L^{(l)}(x)_{i-1}}, 
.., 
\widetilde{ L^{(l)}(x)_{i-4}}
\big] \\
\widetilde{ L^{(l)}(x)_i} &= \sum_{\substack{j \in \llbracket 1 .. M \rrbracket \\ \mathcal{T}(j) = i}} {L^{(l)}(x)_j}, \quad \forall i \in  \llbracket 1 .. N \rrbracket  \\
\mathcal{T} : \llbracket 1 .. M \rrbracket & \rightarrow \llbracket 1 ..  N \rrbracket \\
j & \mapsto i \quad / \quad | t_{y_i} - t_{x_j} | = \min_{k \in [1..N]} | t_{y_k} - t_{x_j} |
\end{align}



with 

\begin{itemize}
    \item \(V\) the set of vocabulary words
    \item \(x = (x_1, .. , x_M) = (\mathrm{once}, \mathrm{upon}, ..., \mathrm{end.}) \in V^M\) the M words of the story.
    \item \(y^{(s)} = (y_1^{(s)}, .., y_N^{(s)}\) the $N$ fMRI scans of one subject $s \in \mathcal{S}$
    \item \(t_x = (t_{x_1}, .., t_{x_M}) \in \bbR^M\)  the $M$ words' onsets and \(t_y = (t_{y_1}, .., t_{y_N})\) ) the timings of the $N$ scan measurements, with respect to the beginning of the experiment.
    \item \(\quad L^{(l)} : x=(x_1, .., x_M) \mapsto L^{(l)}(x) = \big( L^{(l)}(x)_1, .., L^{(l)}(x)_M \big) \in \bbR^{M \times d}\) the application that associates to one text $x$ the elicited GPT2 activations of dimension $M \times d$ (one vector of dimension $d$ per input word), extracted from the layer $l$ of the network  ($l \in \llbracket 0, 12 \rrbracket$). 
    \item \(\mathcal{L} : (x, y) \mapsto \mathrm{Pearsonr}(x, y) \)
\item  $f$ a fitted estimator

==> intro_old.tex <==

%Can we decompose the language representations of vectorial systems? 

% This question is all the more challenging that:
% \begin{itemize}
%     \item In neuroscience, a common way of investigating language processing is to compare the brain activity elicited by two different controlled stimuli (e.g syntactically correct and incorrect sentences) [REF]. Due to the recording and time constraints of neuroimaging, the set of hypotheses that can be tested in one experiment is limited. Thus, different (and therefore heterogeneous) experiments focused on the neural bases of lexico-semantics [REF], compositional-syntax [REF], sentences semantics [REF], but only a few combined these different linguistic dimensions [REF]. 
%     \item More than the experimental setting, one faces a taxonomic obstacle when tackling the question of language processing in the brain. The concepts introduced by linguistic theories vary in the literature and mostly rely on symbolic representations (e.g. tree-like structures), which are difficult to linearly map onto brain activity [REFORMULER?]. Thus, symbols have to be (//are usually) transformed into vectors [XXX], which can have a significant influence on the experimental result [XXX] and hinder its interpretation.
%     \item [REMOVE?] In Natural Language Processing, disentangling linguistic representations is useful to increase its interpretability [XXXX PRECISER VAGUE], better control its biases [XXX FAUX?], but also to build better-performing models (e.g building semantic representations of sentences XXXX STS ?). 
%     \item [REMOVE?] Finally, Linguistics XXX
% \end{itemize}

==> mapping_old.tex <==
\section{Mapping GPT2 activations onto the brain}

% JR proposed order
%{\color{red}

We aim to compare the activations of two systems $\Psi_1$ and $\Psi_2$ input with the same words $w$. $\Psi_1(w)=X\in \mathcal{R}^{M\times d_x}$ refers to GPT2's activations at each of the $M$ word and $\Psi_2(w)=Y\in \mathcal{R}^{N\times d_y}$ refers to the observable brain responses at each of the $N$ fMRI recorded time sample (TR=2\,s). 

To this end, we evaluate a linear spatio- ($f$) temporal ($g$) encoding model trained to predict the $i$\textsuperscript{th} fMRI volume at each voxel $j$, given the network’s activations at the k\textsuperscript{th} layer:

% R=General risk equation
\begin{align} \label{encoding_a}
\mathcal{R}^{(j)}(X) : f^{(j,k)}
\mapsto \mathcal{L} 
\bigg( 
    f^{(j,k)} \circ g(X^{(k)})_{i \in I}, 
    y_{i \in I}^{(j)}
    \bigg)
\end{align}

%In practice, with compute the risk for $x = a^{(k)}(w)$, with $w$ a story and $a^{(k)} : w \in \mathcal{V}^M \mapsto a^{(k)}(w) = [a^{(k)}(w)_1, \dots, a^{(k)}(w)_M] \in \bbR^{M \times d}$ the applications that associate the activations of the layer $k$ of GPT2. This is a measure of the  mapping between the network's activation and one fMRI voxel. We will call this score the "brain score" of one feature space. For simplicity, we will note  $\mathcal{R}(a^{(k)})$ the brain score measured on all the stories $w$ of the stimuli.


% Y=Average BOLD measurement across subjects
Specifically, given a story $w$ of $M$ words ($w = (w_1,  \dots  , w_M) = (\mathrm{the}, \mathrm{cat}, \mathrm{is}, \mathrm{on}, \mathrm{the}, \mathrm{mat} ,\dots \mathrm{end})$, we first extract the corresponding brain measurements $y^{(j)}$ of length $N$ time samples, for the $j$\textsuperscript{th}fMRI. 
To maximize signal-to-noise ratio, we average voxels' responses across the subjects that listened to that story:

\begin{align*}
y^{(j)} & = \Big(
\frac{1}{|\mathcal{S}|} \sum_{s \in \mathcal{S}} \widetilde{y_i}^{(s,j)}
\Big)_{i \in I}
\end{align*}

with 
\(\widetilde{y}^{(s)} = (\widetilde{y_1}^{(s)},  \dots , \widetilde{y_N}^{(s)})\), the $N$ fMRI scans of one subject $s \in \mathcal{S}$, elicited by the story $w$. 

% X=GPT2 activations
We then extract the activations of GPT2 input with the same story $w$. Each of its $k\in \llbracket 0, 12\rrbracket$ layers (from its first "word-embedding" layer ($k=0$) up to its prediction layer ($k=12$)), generates $d_k$ activation values at each word:

\begin{align*}
\Psi_1^{(k)} : \mathcal{V}^M & \rightarrow \bbR^{M \times d} \\
w & \mapsto \Psi_1^{(k)}(w) = [\Psi_1^{(k)}(w)_1, \dots, \Psi_1^{(k)}(w)_M]
\end{align*}

with $\mathcal{V}$ the set of vocabulary words. We note $X^{(k)}$ the activations of layer $k$ elicited by the concatenation of the 27 stories of the stimuli. 

% g: temporally alignment, via FIR+summation
The sampling frequency of bold response is lower than word rate. Furthermore, fMRI signals are associated with delayed time responses that can span several seconds. Following others [refs], we thus align the GPT2's activations to the dynamics of the fMRI responses by applying a finite impulse response (FIR) model $g$.

Specifically, for each fMRI time sample $i \in [1 \dots N]$, $g_i$ combine word features within each TR as follows:
\begin{align*}\label{equ_align}
    g_i : \bbR^{M \times d} & \rightarrow  \bbR^{5d} \\
    u  & \mapsto 
    \big[ 
    \widetilde{ u_i}, 
    \widetilde{ u_{i-1}}, 
    \dots , 
    \widetilde{ u_{i-4}}
    \big] \\
    \widetilde{ u_i} &= \sum_{\substack{m \in \llbracket 1  \dots  M \rrbracket \\ \mathcal{T}(m) = i}} {u_m} \\
\end{align*}
with

\begin{align*}
\mathcal{T} : \llbracket 1  \dots  M \rrbracket & \rightarrow \llbracket 1  \dots   N \rrbracket \\
m & \mapsto i \quad / \quad | t_{y_i} - t_{x_j} | = \min_{k \in \llbracket1 \dots N\rrbracket} | t_{y_k} - t_{x_m} |
\end{align*}

with $\tilde u$ the summed activations of words between successive fMRI time samples, and $u$ the five lags of FIR features.

% f: spatial alignement
Finally, for each layer and each voxel independently, we learn a "spatial" mapping $f^{(j,k)} \in \math{R}^{d_k}$ from the zero-mean unit-variance GPT2 activations of layer $k$ to the zero-mean unit-variance fMRI recordings in voxel $j$ with a $l2$-regularized "ridge" regression:

\begin{align*}
    \underset{f}{\mathrm{argmin}} \smashoperator[r]{\sum_{i}^{I}} \Big(y_{i} - f^T g(X^{(k)})_i\Big)^2 + \lambda ||f||^2 \\
\end{align*}
with $\lambda$ the regularization factor.

We summarize the mapping with a Pearson correlation score:
\begin{align}
    \mathcal{R}^{(j, k)} = \mathrm{corr}\Big(f^{(j,k)T} g(X^{(k)}), y^{(j)}\Big)
\end{align}
 
In practice, $f \circ g$ was fitted on $I_{train}=$ 99\% of the dataset, and evaluated on $I_{test}=$ 1\% of the left out data. %using $\mathcal{L} = \mathrm{Perasonr}$  similarity function. 
We repeated the procedure 100 times following a 100-folds cross validation setting (i.e $(I_k)_{k \in [1 \dots 100]}$ are disjoints intervals of $[1 \dots N]$). This resulted in 100 scores per voxel, which measure the linear mapping between the brain and GPT2 activations elicited by the same story $x$. We will refer to this score as the \emph{brain score} of an activation space $a^{(k)}$. 

% For the sake of readability, we took the example of one story in equation XXX. In practice, we concatenated the XXX stories $x$, the corresponding brain signals $\overline{y}$, and feature vectors  $ u \circ a^{(k)}(x)$. $\overline{y}$ was therefore a weighted averaged over group of subjects, the number of subjects varying across stories. We then fitted and evaluated the estimator on the concatenated features and brain signals. 

%To focus on the specificity of \textit{language} processing in the brain, over speech or auditory processing, we regressed out potential auditory confounds from $\overline{y}$ before fitting $f$. More precisely, for each train fold $I_{train}$ we fitted a ridge linear regression to predict $\overline{y}$ given three types of phonological features (word rate, phoneme rate and phonemes, cf Methods for more details). We then fitted the linear estimator $f$ and computed the associated risk $\mathcal{R}_f$ on the residuals, instead of the full signal $\overline{y}$.

==> old.tex <==

% EQUATIONS
% R=General risk simplified:
\begin{align} \label{encoding_a}
\mathcal{R}^{(k)}(w) : f^{(k)}
\mapsto \mathcal{L} 
\bigg( 
    f^{(k)} \circ g(X^{(k)})_{i \in I}, 
    Y_{i \in I}
    \bigg)
\end{align}


% R=General risk with a:
\begin{align} \label{encoding_a}
\mathcal{R}(x) : f
\mapsto \mathcal{L} 
\bigg( 
    f \circ g(x)_{i \in I}, 
    y_{i \in I}
    \bigg)
\end{align}

% MAPPING





%And the corresponding variance of brain activity explained by syntax is defined by: 
%

%\begin{equation}\label{eq_syn}
%\mathcal{R}(\overline{\psi})
%\end{equation}
%

%Note that we could also first extract the syntactic representations from the network (by taking the E(w)), and then computing the corresponding brain explained variance (R(E(w)). This method, here defined in the case of language processing, can be applied to other types of controls can be applied to embed the syntactical graph in deep neural networks activations. 

 %Note about the assumption that sentences are IID with esperance alpha 

\section{Mapping GPT2 activations onto brain activity }

In the following section, we aim to decompose the brain activity of XXX subjects reading narratives,  into their lexical, compositional, syntactic and semantic components. To this aim, we first factorize the activations of GPT2, a high-performing deep neural language model, and then linearly map the activations, elicited by the subjects' narratives, onto the fMRI brain signals. 

%decompose the activations of two systems $\Psi_1$, a neural network, and $\Psi_2$, the brain, into their lexical, compositional, syntactic and semantic components. Here, $\Psi_1$ refers to GPT2, a high-performing neural language model trained to predict a word given its previous context, on millions of Wikipedia examples. $\Psi_2$ refers to 


%It is comprised of 12 Transformer (contextual) layers ($l \in [1\dots12]$) stacked over a (non-contextual) embedding layer ($l=0$). 

%We study the activations of GPT2, a high-performing neural language models trained to predict a word given its previous context, on millions of Wikipedia example.  


\subsection{Neural language models}
Here, $\Psi_1$ refers to GPT2, a high-performing neural language models trained to predict a word given its previous context, on millions of Wikipedia examples. It is comprised of 12 Transformer (contextual) layers ($l \in [1\dots12]$) stacked over a (non-contextual) embedding layer ($l=0$). 
More precisely, we can define:

\begin{align*}
\Psi_1^{(l)} : \mathcal{V}^M & \rightarrow \bbR^{M \times d} \\
w & \mapsto \Psi_1^{(l)}(w) = [\Psi_1^{(l)}(w)_1, \dots, \Psi_1^{(l)}(w)_M]
\end{align*}

the application that associate to a sequence of words $(w1, \dots, w_)$, the a vector of dimension, for each word, 

We note $X^{(l)}=\Psi_1^{(l)}(w)\in \mathcal{R}^{M\times d_x}$ the activations extracted from layer $l$ elicicite 

First, using the method introduced in section XXX we can split, for each layer $l$, the GPT2 activations $X^{(l)}$ into their syntactic and non syntactic part. We note $\overline{X^{(l)}}$ the syntactic embedding extracted from $X^{(l)}$. Following the definitions introduced in section XXXX, we can decompose $X$ into its:

\begin{itemize}
\item lexical representations : $X^{(0)}$, the word embedding of the network
\item (strictly) compositional representations : $X^{(9)} - X^{(0)}$  i.e the compositional representations $X^{(9)}$, when removing its lexical components. 
\item syntactic representations : $\overline{X^{(l)}}$, that can be extracted for any layer $l \in [0\dots12]$. The \textit{lexical} syntactic representations $\overline{X^{(0)}}$  is actually equivalent to the part-of-speech of the word. Compositional syntactic representations can be extracted from any layer $l>1$ that encode syntactic information. Intermediate layers have been shown to better encode syntactic properties than input and output layers [REF], we therefore consider $\overline{X^{(9)}} = \Psi_1^{(9)}(w)$ as the compositional and syntactic representation of $\Psi_1$. 
\item semantic representations: $X^{(l)} - \overline{X^{(l)}}$, as the residuals of syntactic representations. They can be defined at both the lexical $X^{(0)} - \overline{X^{(0)}}$ and compositional level $X^{(9)} - \overline{X^{(9)}}$.


\subsection{Mapping GPT2 activations onto the brain}
To this aim, we compare the activations of two systems $\Psi_1$, a neural language model, and $\Psi_2$, the brain, when input with the same words $w$ (e.g "not very happy"), and decompose their activations into their lexical, compositional, syntactic and semantic components. 

$\Psi_1^{(l)}(w)=X^{(l)}\in \mathcal{R}^{M\times d_x}$ refers to the activations of the layer $l$ of GPT2, at each of the $M$ words, and $\Psi_2(w)=Y\in \mathcal{R}^{N\times d_y}$ refers to the observable brain responses at each of the $N$ fMRI recorded time sample (TR=2\,s). 


To this end, we evaluate a linear spatio- ($f$) temporal ($g$) encoding model trained to predict the $i$\textsuperscript{th} fMRI volume at each voxel $j$, given the network’s activations at the k\textsuperscript{th} layer:

% R=General risk equation
\begin{align} \label{encoding_a}
\mathcal{R}^{(j, k)}(w) : f^{(j,k)}
\mapsto \mathcal{L} 
\bigg( 
    f^{(j,k)} \circ g(X^{(k)})_{i \in I}, 
    y_{i \in I}^{(j)}
    \bigg)
\end{align}

% R=General risk simplified:
\begin{align} \label{encoding_a}
\mathcal{R}^{(k)}(w) : f^{(k)}
\mapsto \mathcal{L} 
\bigg( 
    f^{(k)} \circ g(X^{(k)})_{i \in I}, 
    Y_{i \in I}
    \bigg)
\end{align}


% R=General risk with a:
\begin{align} \label{encoding_a}
\mathcal{R}(x) : f
\mapsto \mathcal{L} 
\bigg( 
    f \circ g(x)_{i \in I}, 
    y_{i \in I}
    \bigg)
\end{align}

In practice, with compute the risk for $x = a^{(l)}(w)$, with $w$ a story and $a^{(l)} : w \in \mathcal{V}^M \mapsto a^{(l)}(w) = [a^{(l)}(w)_1, \dots, a^{(l)}(w)_M] \in \bbR^{M \times d}$
the applications that associate the activations of the layer $l$ of GPT2. This is a measure of the  mapping between the network's activation and one fMRI voxel. We will call this score the "brain score" of one feature space. For simplicity, we will note  $\mathcal{R}(a^{(l)})$ the brain score measured on all the stories $w$ of the stimuli.


% Y=Average BOLD measurement across subjects
Specifically, given a story $w$ of $M$ words ($w = (w_1,  \dots  , w_M) = (\mathrm{the}, \mathrm{cat}, \mathrm{is}, \mathrm{on}, \mathrm{the}, \mathrm{mat} ,\dots \mathrm{end})$, we first extract the corresponding brain measurements $y^{(j)}$ of length $N$ time samples, for the $j$\textsuperscript{th}fMRI. 
To maximize signal-to-noise ratio, we average voxels' responses across the subjects that listened to that story:

\begin{align}
y^{(j)} & = \Big(
\frac{1}{|\mathcal{S}|} \sum_{s \in \mathcal{S}} \widetilde{y_i}^{(s,j)}
\Big)_{i \in I}
\end{align}

with 
\(\widetilde{y}^{(s)} = (\widetilde{y_1}^{(s)},  \dots , \widetilde{y_N}^{(s)})\), the $N$ fMRI scans of one subject $s \in \mathcal{S}$, elicited by the story $w$. 

% X=GPT2 activations
We then extract the activations of GPT2 input with the same story $w$. Each of its $k\in \llbracket 0, 12\rrbracket$ layers (from its first "word-embedding" layer ($k=0$) up to its prediction layer ($k=12$)), generates $d_k$ activation values at each word:

\begin{align}
X^{(k)} : \mathcal{V}^M & \rightarrow \bbR^{M \times d} \\
w & \mapsto a^{(k)}(w) = [a^{(k)}(w)_1, \dots, a^{(k)}(w)_M]
\end{align}

with $\mathcal{V}$ the set of vocabulary words

% g: temporally alignment, via FIR+summation
The sampling frequency of bold response is lower than word rate. Furthermore, fMRI signals are associated with delayed time responses that can span several seconds. Following others [refs], we thus align the GPT2's activations to the dynamics of the fMRI responses by applying a finite impulse response (FIR) model $g$.

Specifically, for each fMRI time sample $i \in [1 \dots N]$, $g_i$ combine word features within each TR as follows:
\begin{align}\label{equ_align}
    g_i : \bbR^{M \times d} & \rightarrow  \bbR^{5d} \\
    z  & \mapsto 
    \big[ 
    \widetilde{ z_i}, 
    \widetilde{ z_{i-1}}, 
    \dots , 
    \widetilde{ z_{i-4}}
    \big] \\
    \widetilde{ z_i} &= \sum_{\substack{m \in \llbracket 1  \dots  M \rrbracket \\ \mathcal{T}(m) = i}} {z_m} \\
\end{align}
with

\begin{align*}
\mathcal{T} : \llbracket 1  \dots  M \rrbracket & \rightarrow \llbracket 1  \dots   N \rrbracket \\
m & \mapsto i \quad / \quad | t_{y_i} - t_{x_j} | = \min_{k \in \llbracket1 \dots N\rrbracket} | t_{y_k} - t_{x_m} |
\end{align*}

with $\tilde z$ the summed activations of words between successive fMRI time samples, and $z$ the five lags of FIR features.

% f: spatial alignement
Finally, for each layer and each voxel independently, we learn a "spatial" mapping $f^{(j,k)} \in \math{R}^{d_k}$ from the zero-mean unit-variance GPT2 activations of layer $k$ to the zero-mean unit-variance fMRI recordings in voxel $j$ with a $l2$-regularized "ridge" regression:

\begin{align}
    \underset{f}{\mathrm{argmin}} \smashoperator[r]{\sum_{i}^{I}} \Big(y_{i} - f^T g(X^{(k)})_i\Big)^2 + \lambda ||f||^2 \\
\end{align}
with $\lambda$ the regularization factor.

We summarize the mapping with a Pearson correlation score:
\begin{align}
    \mathcal{R}^{(j, k)} = \mathrm{corr}\Big(f^{(j,k)T} g(X^{(k)}), y^{(j)}\Big)
\end{align}

\subsection{Cross-validation}

}

% old version
% \definecolor{grey}{rgb}{0.5, 0.5, 0.5}
% {\color{grey}
% To assess the mapping between the activations of neural language models and the brain, we used, following previous work, a linear encoding setting that predicts the fMRI signals given the network’s activations. More precisely, given a story $x = (x_1, … x_M)$ of $M$ words (e.g. "the", "cat", "is", "on", "the", "mat"), we extracted, for each fMRI voxel: 
% (i)  $\overline{y}$ , the corresponding brain measurements $(y_1, …, y_N)$of length $N$ averaged across the subjects that listened to the story $x$ (we have $N$ MRIs, volumes recorded every 1.5\,s). 
% (ii) the activations of GPT2 when processing the same story $x$. GPT2 is a hierarchical model, composed of stacked Transformer modules, called “layers”, which output one activation vector per token, from its first embedding layer ($l=0$) to the output layer ($l=12$). Therefore, for each layer $l$, the activation vector elicited by the story $x$ is of dimension $(M, d)$, hereafter noted $a^{(l)}(x)$.  
% There are more words than fMRI recordings, and the BOLD measurement is delayed compared to the brain response. To align the two time domains,  the alignment function $u$ (cf equation XXX) sums the (word-timed) features occurring between each fMRI measurement and concatenate the summed vectors using a finite impulse response (FIR) model [REF]. Thus, after applying $u$, we obtain one feature vector $u_i \circ a^{(l)}(x)$ per fMRI measurement $\overline{y}_i$, $i \in [1 \dots N]$.

% Then, an estimator is fitted to map the neural network activations $\big(u_i \circ a^{(l)}(x)\big)_{i \in I_{train}}$ onto  the brain activations $(\overline{y}_i)_{i \in I_{train}}$, given an interval $I_{train} \subset [1 \dots N]$). Finally, the empirical risk of the fitted estimator can be assessed by computing the similarity function $\mathcal{L}$ between predicted and actual brain measurements over an interval $I \subset I$, as follows:

% \input{equations}

==> old_abstract.tex <==
 % otherwise use the standard text.

% \begin{abstract}

% % JR's proposal
% The structure of sentences follows a latent hierarchical organization. This so-called "syntax", according to linguistics, can be incrementally built by a recursive operator, whose precise nature, however, remains notoriously unknown.
% Here, we introduce a simple method to factorize the operations of a neural language model -- GPT2 -- into four types of representations: lexical, compositional, syntactic, and semantic representations. We then use this method to decompose the brain responses of 345 subjects recorded with functional magnetic resonance imaging (fMRI) during the listening of ~4.6 hours of narrated text, and successfully map GPT2's factorized activations onto those of the brain. 
% %
% % results
% % Ce serait mieux de ne pas mettre les resultats mais une ouverture non ? 
% ((Compositional processing was revealed to be more distributed and right-lateralized than lexical processing. Semantic representations were more frontal than syntactic ones, but both lied in a shared network. ))
% %
% % conclusion / opening
% These results isolate the brain networks associated with the generation of compositional structures and meaning during natural speech processing.


% \end{abstract}
